Fixed-Order H-Infinity Controller Design for Port-Hamiltonian Systems

We present a new fixed-order H-infinity controller design method for potentially large-scale port-Hamiltonian (pH) plants. Our method computes controllers that are also pH (and thus passive) such that the resulting closed-loop systems is again passive, which ensures closed-loop stability simply from the structure of the plant and controller matrices. In this way, we can avoid computationally expensive eigenvalue computations that would otherwise be necessary. In combination with a sample-based objective function which allows us to avoid multiple evaluations of the H-infinity norm (which is typically the main computational burden in fixed-order H-infinity controller synthesis), this makes our method well-suited for plants with a high state-space dimension. In our numerical experiments, we show that applying a passivity-enforcing post-processing step after using well-established H-infinity synthesis methods often leads to a deteriorated H-infinity performance. In constrast to that, our method computes pH controllers, that are automatically passive and simultaneously aim to minimize the H-infinity norm of the closed-loop transfer function. Moreover, our experiments show that for large-scale plants, our method is significantly faster than the well-established fixed-order H-infinity controller synthesis methods.

==> performance_table.tex <==
$ $Plant & order & SOBMOR & hifoo & hinfstruct & hifoo\_passive & hinfstruct\_passive \\ 
EB1 & 1 &  3.105e+00 & 3.114e+00 & 3.105e+00 & 3.114e+00 & 3.105e+00 \\
EB1 & 2 &  3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 \\
EB1 & 3 &  3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 & 3.107e+00 \\
EB1 & 4 &  3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 \\
EB1 & 5 &  3.104e+00 & 3.104e+00 & 3.104e+00 & 3.104e+00 & 3.105e+00 \\\hline 
EB2 & 1 &  1.809e+00 & 1.800e+00 & 2.020e+00 & 1.800e+00 & 2.020e+00 \\
EB2 & 2 &  1.786e+00 & 1.782e+00 & 1.800e+00 & 1.374e+01 & 1.801e+00 \\
EB2 & 3 &  1.782e+00 & 1.777e+00 & 1.780e+00 & 1.784e+00 & 1.848e+00 \\
EB2 & 4 &  1.781e+00 & 1.776e+00 & 1.776e+00 & 1.841e+00 & 1.779e+00 \\
EB2 & 5 &  1.781e+00 & 1.776e+00 & 1.780e+00 & 1.938e+00 & 3.891e+00 \\\hline 
EB3 & 1 &  1.906e+00 & 1.906e+00 & 2.057e+00 & 1.906e+00 & 2.057e+00 \\
EB3 & 2 &  1.866e+00 & 1.866e+00 & 1.905e+00 & 1.866e+00 & 1.905e+00 \\
EB3 & 3 &  1.829e+00 & 1.818e+00 & 1.819e+00 & 2.043e+00 & 1.893e+00 \\
EB3 & 4 &  1.816e+00 & 1.813e+00 & 1.819e+00 & 2.455e+00 & 1.819e+00 \\
EB3 & 5 &  1.813e+00 & 1.805e+00 & 1.818e+00 & 2.361e+00 & 4.694e+00 \\\hline 
EB4 & 1 &  1.905e+00 & 1.905e+00 & 2.056e+00 & 1.905e+00 & 2.056e+00 \\
EB4 & 2 &  1.865e+00 & 1.865e+00 & 1.901e+00 & 1.865e+00 & 1.901e+00 \\
EB4 & 3 &  1.829e+00 & 1.818e+00 & 1.818e+00 & 2.064e+00 & 1.890e+00 \\
EB4 & 4 &  1.816e+00 & 1.814e+00 & 1.820e+00 & 2.357e+00 & 7.440e+00 \\
EB4 & 5 &  1.813e+00 & 1.805e+00 & 1.818e+00 & 2.373e+00 & 2.070e+00 \\\hline 
EB5 & 1 &  1.905e+00 & 1.905e+00 & 1.964e+00 & 1.905e+00 & 1.968e+00 \\
EB5 & 2 &  1.865e+00 & 1.865e+00 & 1.902e+00 & 1.865e+00 & 1.903e+00 \\
EB5 & 3 &  1.829e+00 & 1.818e+00 & 1.846e+00 & 2.467e+00 & 1.847e+00 \\
EB5 & 4 &  1.816e+00 & 1.812e+00 & 1.818e+00 & 2.458e+00 & 2.541e+00 \\
EB5 & 5 &  1.813e+00 & 1.805e+00 & 1.817e+00 & 5.247e+00 & 8.130e+00 \\\hline 
EB6 & 1 &  1.905e+00 & 1.905e+00 & 1.905e+00 & 1.905e+00 & 1.905e+00 \\
EB6 & 2 &  1.865e+00 & 1.865e+00 & 1.903e+00 & 1.865e+00 & 1.903e+00 \\
EB6 & 3 &  1.829e+00 & 1.818e+00 & 1.818e+00 & 1.906e+00 & 2.522e+00 \\
EB6 & 4 &  1.816e+00 & 1.812e+00 & 1.818e+00 & 4.153e+02 & 5.124e+00 \\
EB6 & 5 &  1.813e+00 & 1.809e+00 & 1.818e+00 & 2.859e+00 & 2.184e+00 \\\hline 
DLR1 & 1 &  1.366e+00 & 6.666e-01 & 2.776e+00 & 6.666e-01 & 2.776e+00 \\
DLR1 & 2 &  5.097e-01 & 2.430e-01 & 2.430e-01 & 6.389e+00 & 5.022e+00 \\
DLR1 & 3 &  4.682e-01 & 2.055e-01 & 2.208e-01 & 4.404e+00 & 6.743e+00 \\
DLR1 & 4 &  4.397e-01 & 7.413e-02 & 7.564e-02 & 6.887e+00 & 4.056e+00 \\
DLR1 & 5 &  3.813e-01 & 7.074e-02 & 1.427e-01 & 5.221e+00 & 1.427e-01 \\\hline 
LAH & 1 &  5.373e-05 & 5.373e-05 & 5.373e-05 & 5.373e-05 & 5.373e-05 \\
LAH & 2 &  5.373e-05 & 5.373e-05 & 5.373e-05 & 5.373e-05 & 5.373e-05 \\
LAH & 3 &  5.373e-05 & 5.373e-05 & 5.373e-05 & 1.426e-02 & 5.373e-05 \\
LAH & 4 &  5.373e-05 & 5.373e-05 & 5.373e-05 & 1.314e-01 & 5.373e-05 \\
LAH & 5 &  5.373e-05 & 5.373e-05 & 5.373e-05 & 2.932e-03 & 5.373e-05 \\\hline 
NN18 & 1 &  1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 \\
NN18 & 2 &  1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 \\
NN18 & 3 &  1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 \\
NN18 & 4 &  1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 \\
NN18 & 5 &  1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 & 1.000e-02 \\\hline 

